Fast Generation of Custom Floating-Point Spatial Filters on FPGAs

Convolutional Neural Networks (CNNs) have been utilised in many image and video processing applications. The convolution operator, also known as a spatial filter, is usually a linear operation, but this linearity compromises essential features and details inherent in the non-linearity present in many applications. However, due to its slow processing, the use of a nonlinear spatial filter is a significant bottleneck in many software applications. Further, due to their complexity, they are difficult to accelerate in FPGA or VLSI architectures. This paper presents novel FPGA implementations of linear and nonlinear spatial filters. More specifically, the arithmetic computations are carried out in custom floating-point, enabling a tradeoff of precision and hardware compactness, reducing algorithm development time. Further, we show that it is possible to process video at a resolution of 1080p with a frame rate of 60 frames per second, using a low-cost FPGA board. Finally, we show that using a domain-specific language will allow the rapid prototyping of image processing algorithms in custom floating-point arithmetic, allowing non-experts to quickly develop real-time video processing applications.

==> overview_framework.tex <==
\section{Proposed Floating-point Library}\label{sec:overview_framework}
This section gives an overview the proposed architectures and implementation of the floating-point library. Subsection \ref{subsec:fp_conversion} describes conversion between floating-point and fixed-point. Subsection \ref{subsec:add_mult} covers the implementation of the floating-point adder and multiplier and subsection \ref{subsec:poly_functions} discusses the implementation and architectures of the functions (division, logarithm, square-root and exponentiation) based on the polynomial approximation. 

\subsection{Conversion between floating-point and fixed-point}\label{subsec:fp_conversion}
Let $x$ and $X$ be the representations of a floating-point and a fixed-point number, respectively. According to equation \ref{eq:fp_reps}, $x$ is a function of the sign $s$, the exponent $e$ and the mantissa $m$. On the other hand, $X$ is a function of $M$ integer bits, $N$ fractional bits, where $a_k$ and $b_k \in \{0,1\}$ and $X$ also is represented in 2's complement, i.e., $(-X)=2^{M+N+1}-X$.

\begin{figure*}[h]
    \centering 
    %\includegraphics[width=\columnwidth]{img/FP_fix.pdf}
    \includegraphics[width=\linewidth]{img/fplib_basic.pdf}
    \caption{Architectural descriptions of the floating-point adder, multiplier and conversion between floating-point to fixed-point.}
    \label{fig:fplib_basic}
\end{figure*}

\begin{equation}\label{eq:fp_reps}
\left\{\begin{matrix}
x = (-1)^s\times2^e\times1.m\\ 
X = \sum \limits_{k=0}^{M}a_k2^{N+k}+\sum \limits_{k=1}^{N}b_k2^{N-k}
\end{matrix}\right.
\end{equation}

Let $\chi: x\rightarrow X$ be a function to convert a floating-point to a fixed-point number. $\chi$ can be defined as $X = \chi(x) = x\times 2^N$. The implementation of $\chi$ is a shift of the mantissa with $e+N$ bits. Similarly, let  $\chi^{-1}: X\rightarrow x$ be a fucntion to convert a fixed-point to a floating-point number. The determination of $\chi^{-1}$ is done by finding the most signifcant bit (MSB) of $X$ using a leading-one detector to compute the exponent. After finding the exponent, the mantissa is computed truncating $X$ to its MSB position. An overview of the architectures to computer $\chi$ and $\chi^{-1}$ is shown in figure \ref{fig:fplib_basic}. Note that the determination of the signs of $x$ and $X$  is done by checking if the bit $s=a_M$ is zero (positive) or one (negative).

\subsection{Floating-point adder and multiplier}\label{subsec:add_mult}
Given two floating-point numbers $x=(-1)^{s_x}\times2^{e_x}\times1.m_x$ and $y=(-1)^{s_y}\times2^{e_y}\times1.m_y$, if $|x|\geq |y|$, than $x\pm y$ has the form of the equation \ref{eq:add_sub}. 

\begin{equation}\label{eq:add_sub}
x\pm y = (-1)^{s_x}\times \left(1.m_x\pm \frac{1.m_y}{2^{e_x-e_y}}\right) \times2^{e_x}
\end{equation}

The steps required to compute $x\pm y$ is described as follows. The first step is to swap $x$ and $y$ if $|y| > |x|$. This guarantees that $|x|\geq |y|$ and that the expression $e_x-e_y$ will always be positive. The next step is to shift the mantissa of the smallest number with the exponent difference and add the shifted mantissa to the mantissa of the bigger number. Finally, a normalisation stage is required to normalise the mantissa (and increment the exponent) of the resulted operation. This is required if the resulted mantissa is smaller than 1. The normalisation stage can be processed using a leading-one detector to find the MSB bit of the mantissa. It is important to note that the hardware implementation of the shift stage can infer barrel shifters and compromise the performance of the floating-point adder \cite{karlstrom2006high}. The high-performance computation can be achieved using pipelined stages in addition to the substitution of the barrel shifts with a set of constant shifts executed in parallel.

Consider now the operation of floating-point multiplication defined in the equation \ref{eq:mult}. 

\begin{equation}\label{eq:mult}
x\times y=(-1)^{s_x \oplus s_y}\times 2^{e_x+e_y}\times(1.m_x\times 1.m_y)
\end{equation}

The floating-point multiplication is straightforward. The sign of the product is the xor operation of the sign operands. The exponent and mantissa of the product consist of the sum and multiplication of the exponent and mantissae of the operands, respectively. Similar to the addition, the normalisation of the mantissa (and the descrease of the exponent) is also required if the resulted mantissa is bigger than 1. The basic architectural description of the floating-point adder and multiplier is also shown in figure \ref{fig:fplib_basic}.

\subsection{Polynomial approximation based functions}\label{subsec:poly_functions}
The implementation of a floating-point divider is conceptually similar to the multiplication operation.  According to equation \ref{eq:div}, the computation of the quotient's sign also results from a xor operation.  The exponent of the quotient is the difference of the operand exponents, and the mantissa is the product of the mantissa's dividend with the reciprocal of the mantissa's divisor. In addition to that, an exception handling deals with division by zero, infinities and not-a-numbers. However, the computation of the reciprocal of the mantissa turns the divider a complex function.  

\begin{equation}\label{eq:div}
\frac{x}{y}=(-1)^{s_x \oplus s_y}\times 2^{e_x-e_y}\times 1.m_x\times \frac{1}{1.m_y}
\end{equation}

Although a change in the base only adds a constant multiplication, the logarithm in base 2 is the most convenient due to its simplicity. According to equation \ref{eq:log2}, if the operand is negative, the resulted logarithm is not-a-number, since the logarithm is defined only for positive reals. Otherwise, the result is the logarithm of the mantissa added to the shifted exponent of the operand \cite{langhammer2017single}. This addition results in a fixed-point number and a floating-point to fixed-point conversion converts the final value. Additionally, an exception handling can handle operations with infinities and not-a-numbers. 

\begin{equation}\label{eq:log2}
    \log_2(x)=\left\{
                \begin{array}{ll}
                  e+log_2(1.m), &\mbox{if $s=0$}  \\
                  NaN, &\mbox{if $s=1$} 
                \end{array}
              \right.
\end{equation}

The floating-point exponentiation can be simplified by selecting the base 2 for the power function\footnote{Again, the base change is realized with a constant multiplication.}. The first step for the operation is to convert the floating-point to a fixed point number and break the result into two parts $X_I$ and $X_F$ \cite{detrey2005parameterized}. As described in equation \ref{eq:pow2}, the integer number $X_I$ is the resulted exponent. The mantissa is computed with the expression $2^{X_F}$, if the operand $x$ is positive, or $2^{-X_F}$ is if $x<0$.  The exception handling is responsible to manipulate underflows, overflows, infinities and not-a-numbers.

\begin{equation}\label{eq:pow2}
    2^x = 2^{(-1)^s\times(X_I+X_F)}= \left\{
                \begin{array}{ll}
                  2^{X_I}\times 2^{X_F}, &\mbox{if $s=0$}  \\
                  2^{-X_I}\times \frac{1}{2^{X_F}}, &\mbox{if $s=1$} 
                \end{array}
              \right.
\end{equation}

The floating-point square-root operation is defined in equation \ref{eq:sqrt}. The idea is to compute the square-root of the mantissa's operand if its exponent is even or to multiply the mantissa's operand by two and take the square-root if the exponent is odd \cite{de2010multiplicative}. The resulted exponent is calculated checking the least significant bit of the exponent's operand and based on this bit, the exponent is decrement by one, followed by a division by two using a shift register\footnote{If the operand is negative, the resulted square-root is not-a-number.}. The computation of the mantissa requires the implementation of the square-root operand to compute the number $\sqrt{t}$ in the range $t\in [1,4)$.

\begin{equation}\label{eq:sqrt}
    \sqrt{x} = \left\{
                \begin{array}{ll}
                  2^{\frac{e}{2}}\times \sqrt{1.m}, &\mbox{if \textit{e} is even}\\
                  2^{\frac{e-1}{2}}\times \sqrt{2\times 1.m}, &\mbox{if \textit{e} is odd}\\
                  NaN, & \mbox{if $s=1$} 
                \end{array}
              \right.
\end{equation}

The implementation of the operations in equations 1 to 4 requires the manipulation of transcendental functions\footnote{Even the division, not considered a transcendental function, still requires an approximation.}, which can be computed using polynomial approximations within a specific range.  The accuracy of the implementation is dependent on the degree of the polynomial used in the approximation. Slicing the range of the function into smaller segments leads to improved accuracy\cite{lee2008hardware}.

A function $f(x)$ can be approximated by a degree-$d$, $n$-segments polynomial $y$ in the range $x_i\leq x<x_f$. The approximated function in the $k$-th segment is defined according to equation \ref{eq:poly}, where $\eta=\frac{(x_f-x_i)}{n}$ and the matrix $C_{n\times d}$ contains the coefficients of the polynomial approximation. 

\begin{equation}\label{eq:poly}
\begin{matrix}
y(k,d,x) \approx \sum\limits_{n=0}^{d}C(k,n)x^{d-n},&  x_i+k\eta\leq x < x_i+(k+1)\eta
\end{matrix}
\end{equation}

\begin{figure}[h]
    \centering 
    \includegraphics[width=\columnwidth]{img/poly.pdf}
    \caption{Parameterizable degree-$d$, $n$-segments polynomial approximator}
    \label{fig:poly}
\end{figure}

Figure \ref{fig:poly} illustrates the hardware implementation of a general polynomial approximator. The architecture is parameterizable in terms of the degree $d$ and the number of segments $n$. The computation of the approximation uses $d$ additions and $d$ multiplications. Moreover, $n\times(d+1)$ coefficients are stored in lookup tables to evaluate the approximations. 

\begin{figure*}[h]
    \centering 
    %\includegraphics[width=\columnwidth]{img/poly_math.pdf}
    \includegraphics[width=\linewidth]{img/fplib_poly.pdf}
    \caption{Hardware implementation of floating-point division, logarithm, square-root and exponentiation using the general polynomial approximator}
    \label{fig:fplib_poly}
\end{figure*}


\begin{equation}\label{eq:Ca}
C^{\alpha} = \begin{bmatrix}
                 0.70986& -0.9735  & 0.99947\\
                 0.38742& -0.82214 & 0.98109\\
                 0.23424& -0.67285 & 0.94441\\
                 0.15228& -0.55171 & 0.89948
               \end{bmatrix}, I^{\alpha} \in \left[0,1\right )
\end{equation}

\begin{equation}\label{eq:Cb}
C^{\beta} = \begin{bmatrix}
                 -0.573   &  1.42883 &  0.00028\\
                 -0.3829  &  1.33815 &  0.0147\\
                 -0.27387 &  1.2312  &  0.03792\\
                 -0.20558 &  1.12988 &  0.07564
               \end{bmatrix}, I^{\beta} \in \left[0,1\right )
\end{equation}

\begin{equation}\label{eq:Cc}
C^{\gamma} = \begin{bmatrix}
                0.14315 & 0.62811 & 0.98516\\
                0.20244 & 0.68584 & 0.9997\\
                0.28629 & 0.68363 & 1.0004\\
                0.40488 & 0.56192 & 1.0326 
               \end{bmatrix}, I^{\gamma} \in \left[-1,1\right )
\end{equation}

\begin{equation}\label{eq:Cd}
C^{\delta} = \begin{bmatrix}
                 -0.07913 &  0.64644 &  0.43337\\
                 -0.04069 &  0.51676 &  0.54339\\
                 -0.02576 &  0.44338 &  0.63378\\
                 -0.01816 &  0.39451 &  0.71252 
                \end{bmatrix}, I^{\delta} \in \left[1,4\right )
\end{equation}

The hardware implementation of the floating-point operations of division, logarithm, square-root and exponentiation is shown in figure \ref{fig:fplib_poly}. Equations \ref{eq:Ca} to \ref{eq:Cd} show the coefficients and ranges $I\in[x_i, x_f)$ used in the approximations for the operations reciprocal ($\frac{1}{x}$), logarithm ($log_2(x)$), exponentiation ($2^x$) and square-root ($\sqrt{x}$), respectively. A degree-2, 4-segments polynomial is chosen in this particular case. Each function incorporates one instance of the polynomial approximator in its datapath, allowing the generation of customizable hardware with little modification. The latency of the operations is a function of the degree of the polynomials. This results from the pipelined additions and multiplications in the polynomial approximator to achieve high-performance computation. The number of segments does not affect the latency, once the ranges are selected using a combinatorial priority encoder\footnote{Alternatively, the range of $x$ is selected using the $\lceil log_2(n)\rceil$ MSB bits of $x$.}. Table \ref{tab:latency} shows the latency of each floating-point operation described in this work.

\begin{table}[h]
  \caption{Latency and throughput of each floating-point operation}\label{tab:latency}
  \centering
  \begin{tabular}{{|c|c|c|}}
    \hline
    %\hline
    \textbf{Operation} & \textbf{Latency} & \textbf{Throughput}\\
    \hline
    \hline
    float2fix conversion & 1 cycle & 1 operation per cycle\\
    \hline
    fix2float conversion & 1 cycle & 1 operation per cycle\\
    \hline
    addition & 6 cycles & 1 operation per cycle\\
    \hline
    multiplication & 1 cycle & 1 operation per cycle\\
    \hline
    degree-d approx. for division & d+4 cycles & 1 operation per cycle\\ 
    \hline
    degree-d approx. for exponentiation & d+4 cycles & 1 operation per cycle\\
    \hline
    degree-d approx. for logarithm & d+3 cycles & 1 operation per cycle\\
    \hline
    degree-d approx. for square-root & d+3 cycles & 1 operation per cycle\\ 
    %\hline
    \hline
  \end{tabular}
\end{table}

